Learn to explain yourself, when you can: Equipping Concept Bottleneck Models with the ability to abstain on their concept predictions

The Concept Bottleneck Models (CBMs) of Koh et al. [2020] provide a means to ensure that a neural network based classifier bases its predictions solely on human understandable concepts. The concept labels, or rationales as we refer to them, are learned by the concept labeling component of the CBM. Another component learns to predict the target classification label from these predicted concept labels. Unfortunately, these models are heavily reliant on human provided concept labels for each datapoint. To enable CBMs to behave robustly when these labels are not readily available, we show how to equip them with the ability to abstain from predicting concepts when the concept labeling component is uncertain. In other words, our model learns to provide rationales for its predictions, but only whenever it is sure the rationale is correct.

==> 2211 (1).11690/result_tables.tex <==
\begin{table}[h!]
\tiny
\centering
\begin{tabular}{llllll}
\toprule
            & Prob. Missing Concept &              0.00 &              0.25 &              0.50 &              0.75 \\
Dataset Name & Sidecar CLM &                   &                   &                   &                   \\
\midrule
InOutFashionMNIST & False &  $0.988\pm 0.001$ &  $0.975\pm 0.001$ &   $0.97\pm 0.002$ &  $0.873\pm 0.035$ \\
            & True  &  $0.989\pm 0.001$ &  $0.987\pm 0.002$ &  $0.987\pm 0.002$ &  $0.984\pm 0.003$ \\
LivingCIFAR10 & False &  $0.946\pm 0.002$ &  $0.876\pm 0.062$ &  $0.843\pm 0.039$ &  $0.504\pm 0.036$ \\
            & True  &  $0.964\pm 0.002$ &  $0.959\pm 0.001$ &  $0.956\pm 0.001$ &  $0.955\pm 0.002$ \\
ParityMNIST & False &  $0.982\pm 0.002$ &   $0.97\pm 0.001$ &  $0.964\pm 0.009$ &  $0.939\pm 0.006$ \\
            & True  &    $0.987\pm 0.0$ &  $0.985\pm 0.001$ &    $0.988\pm 0.0$ &  $0.986\pm 0.003$ \\
\bottomrule
\end{tabular}
\caption{Average, and standard deviation of accuracy for the target task.}
\label{tab:results1}
\end{table}
\begin{table}[h!]
\tiny
\centering
\begin{tabular}{llllll}
\toprule
            & Prob. Missing Concept &              0.00 &              0.25 &              0.50 &              0.75 \\
Dataset Name & Sidecar CLM &                   &                   &                   &                   \\
\midrule
InOutFashionMNIST & False &     $0.97\pm 0.0$ &  $0.946\pm 0.006$ &   $0.94\pm 0.002$ &  $0.763\pm 0.016$ \\
            & True  &  $0.987\pm 0.001$ &    $0.993\pm 0.0$ &  $0.997\pm 0.001$ &      $1.0\pm 0.0$ \\
LivingCIFAR10 & False &  $0.733\pm 0.002$ &  $0.624\pm 0.008$ &  $0.506\pm 0.021$ &  $0.206\pm 0.066$ \\
            & True  &  $0.908\pm 0.003$ &  $0.936\pm 0.003$ &   $0.97\pm 0.003$ &  $0.948\pm 0.017$ \\
ParityMNIST & False &  $0.967\pm 0.003$ &  $0.943\pm 0.003$ &  $0.925\pm 0.014$ &  $0.878\pm 0.014$ \\
            & True  &  $0.988\pm 0.001$ &  $0.993\pm 0.001$ &  $0.997\pm 0.001$ &      $1.0\pm 0.0$ \\
\bottomrule
\end{tabular}

\caption{Average, and standard deviation of F1 score for explanation accuracy.}
\label{tab:results2}
\end{table}
\begin{table}[h!]
\tiny
\centering
\begin{tabular}{llllll}
\toprule
            & Prob. Missing Concept &             0.00 &             0.25 &             0.50 &             0.75 \\
Dataset Name & Sidecar CLM &                  &                  &                  &                  \\
\midrule
InOutFashionMNIST & False &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ \\
            & True  &  $0.966\pm 0.003$ &  $0.905\pm 0.017$ &  $0.453\pm 0.064$ &  $0.002\pm 0.002$ \\
LivingCIFAR10 & False &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ \\
            & True  &  $0.653\pm 0.059$ &  $0.423\pm 0.013$ &   $0.11\pm 0.025$ &  $0.005\pm 0.005$ \\
ParityMNIST & False &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ &      $1.0\pm 0.0$ \\
            & True  &  $0.963\pm 0.005$ &   $0.88\pm 0.012$ &  $0.419\pm 0.071$ &  $0.001\pm 0.001$ \\
\bottomrule
\end{tabular}
\caption{Proportion of datapoints in test set that the model provided an explanation for. Note that the standard CBM always provides an explanation, so proportion is always $1$.}
\label{tab:results3}
\end{table}
